Concurrency Control as a Service

Existing disaggregated databases separate execution and storage layers, enabling independent and elastic scaling of resources. In most cases, this design makes transaction concurrency control (CC) a critical bottleneck, which demands significant computing resources for concurrent conflict management and struggles to scale due to the coordination overhead for concurrent conflict resolution. Coupling CC with execution or storage limits performance and elasticity, as CC's resource needs do not align with the free scaling of the transaction execution layer or the storage-bound data layer. This paper proposes Concurrency Control as a Service (CCaaS), which decouples CC from databases, building an execution-CC-storage three-layer decoupled database, allowing independent scaling and upgrades for improved elasticity, resource utilization, and development agility. However, adding a new layer increases latency due to the shift in communication from hardware to network. To address this, we propose a Sharded Multi-Write OCC (SM-OCC) algorithm with an asynchronous log push-down mechanism to minimize network communications overhead and transaction latency. Additionally, we implement a multi-write architecture with a deterministic conflict resolution method to reduce coordination overhead in the CC layer, thereby improving scalability. CCaaS is designed to be connected by a variety of execution and storage engines. Existing disaggregated databases can be revolutionized with CCaaS to achieve high elasticity, scalability, and high performance. Results show that CCaaS achieves 1.02-3.11X higher throughput and 1.11-2.75X lower latency than SoTA disaggregated databases.

==> bak.tex <==
%
%
%
%
%
%
%
\section{Introduction}
\label{section:1}

Database systems are redesigned based on a cloud-native architecture, decoupling storage from the system to form a compute-storage two-layer architecture. So that cloud-native databases \cite{loesing2015designtell, das2013elastras, huang2020tidb, zhou2021foundationdb, abadi2003aurora, taft2020cockroachdb, redshift, yang2022oceanbase, thusoo2009hive, yu2020pushdowndb, yang2021flexpushdowndb} can adapt to the cloud environment with disaggregated computing and storage resources and easily scale them independently to achieve good scalability. 
The spirit of cloud-native architecture is decoupling. Cloud provides the elasticity of different decoupled resources (\eg computation, memory, and storage), allowing growing or shrinking the resource capacity to adjust to the changing demands. To achieve excellent elasticity with efficient resource utilization, systems should be decoupled into a number of modules, so that each function module that mainly rely on a specific resource with specific scaling requirements can be scaled independently.
Furthermore, decoupled function modules can be integrated into independent services like cloud storage services \cite{cao2018polarfs, zhu2018solar, awss3, azureblob, googlecloudservice} and cache services \cite{awselasticache, lee2021mind} to develop agility, reliability, and maintainability \cite{alshuqayran2016systematic, cerny2018contextual} applications.


Based on the fact that transaction execution requires a large amount of computational resources and data storage requires a large amount of storage space, most of the existing cloud-native databases adopt a common approach to decouple the system into a compute-storage architecture. 
For instance, TiDB \cite{huang2020tidb} uses the SQL execution engine (TiDB server) to form the compute layer and adopts a distributed key-value (KV) store TiKV \cite{tikv} as the storage layer. The TiDB servers are the stateless engines that receive SQL requests, perform SQL parsing and optimization, generate a distributed execution plan, and do the computation. TiKV acts as an independent KV store and provides transaction ACID properties (atomicity, consistency, isolation, and durability).
The compute layer can be scaled out by adding more nodes to handle the increasing query demands effectively. On the other hand, the storage layer can scale to accommodate the growing data volume. 
Such a design provides flexibility to scale independent resources, promotes modularity and reusability, and is ideal for independent evolution.


\begin{figure}
% \vspace{-0.1in}
  \centerline{\includegraphics[width=0.4\textwidth]{figs/DB components auto crop.pdf}}
  \centering
  % \vspace{-0.05in}
  \caption{An execution-transaction-storage three-layer cloud-native database architecture.}
  \label{fig:DB}
  \vspace{-0.1in}
\end{figure}


However, transaction management (TM), which ensures the transaction ACID properties, has different resource requirements and scaling capabilities between transaction execution and data storage. But, the computation and scaling requirements of TM have been ignored by these databases that simply couple TM with transaction execution or data storage. This lack of sufficient decoupling may lead to performance or scalability problems in the system.


As a key component of the database, TM has limited scalability and requires sufficient computational resources to handle concurrent accesses. 
This is because the concurrency control (CC) algorithm used in concurrency conflict resolution can not scale well due expensive coordination overhead \cite{TheEndofaMyth, thomson2010casedeterminism, stonebraker2018onesizefitsall, ren2012lightweightlocking, kallman2008hstore, curino2010schism}. 
By using the sharding strategy, the workloads to be spread across multiple machines, but introduces a lot of communication overheads that limit the scalability of transaction management.
When coupling TM with transaction execution, the compute layer can be scaled out with more compute nodes to add computation resources. But, using more compute nodes leads to distributed transactions and adds more communication overhead. The coordination overhead will outweigh the benefit of adding more computing resources, and the performance of transaction management drops as the number of nodes increases \cite{zamanian2016end, mahmoud2014maat, salomie2011database}. 


Considering that most existing CC algorithms must handle conflicts of the same data item on a single node, databases like CockroachDB \cite{taft2020cockroachdb}, TiDB \cite{huang2020tidb} \etc couple the TM with the storage layer so that transaction conflicts are handled at the location where the data item belongs. In addition, logs, which is used to ensure transaction persistence (durability), can be store on the storage layer directly.
However, data storage, a massive data access service, requires a large amount of storage space instead of computing resources. The storage layer is often equipped with machines with high-volume SSDs/disks but relatively low computing resources; coupling TM with storage limits transaction management performance.


To achieve efficient transaction management, TM should be equipped with high computation resources for concurrency access, and the number of nodes does not need to be expanded significantly.
Meanwhile, a certain amount of disk storage space is required to store transaction log.


Considering the principle of cloud-native designs (\ie continuously decoupling functionality), it is desirable to decouple TM from the database system to maximize the scalability and elasticity of the database system in the cloud environment. 
Furthermore, by making the decoupled TM work as an independent transaction service, which can be independently upgraded and evolved, the TM service can promote development agility and adaptability for the database system.



In this paper, we propose \textbf{\emph{Transaction as a Service} (TaaS)}, a concept aimed at decoupling a separate transaction management layer and making it work as a service to build an execution-transaction-storage three-layer cloud-native database as shown in Figure \ref{fig:DB}. The execution layer executes the transaction requests, reads data from data storage, and send transaction management requests to the TaaS layer for concurrent concurrency control. TaaS handles transaction concurrent conflicts and logs the successfully committed transactions. Then, the commit/abort notifications are returned to the execution layer, and the transaction logs are sent to the storage layer to update the data.


As a service, TaaS is designed to be connected by multiple data model execution engines with various data models (including KV, relational, graph, \etc). To be invoked by multiple execution engines simultaneously, we define a unified interface to support the invocation of many different model engines for the transaction management service.  Since the transaction management focuses on read and write conflict resolution on data items and cares nothing about the data processing and storage location. By abstracting the accessed read and write sets logically, we can avoid the influence of the data models on transaction management. 
Using TaaS, the execution layer can consist of multiple execution engines that execute transactions and send transaction management requests to TaaS.


To ensure high availability of the transaction management service, TaaS needs to be up and running even when some of the TaaS nodes fail. However, in a master-followers architecture, the backup machine takes some time to recover when the master node fails, making the system temporarily unavailable. Thus, TaaS adopts a multi-master architecture where multiple master nodes work together to provide transaction management services. Moreover, TaaS adopts a sharding mechanism to provide a certain degree of scalability for the system. The TaaS requirements will be discussed in detail in Section \ref{subsection:Requirements}.


TaaS is dedicated to resolve transaction conflicts and adpots an Epoch-based Sharded Multi-Master OCC algorithm (Section \ref{subsection:Transaction Management}). After completing conflict handling, TaaS updates transactions that win in conflict resolution to the storage layer. When connecting to multiple execution engines, TaaS needs to support connecting to heterogeneous storage engines and updating data. One of the most important things is to ensure the transaction atomic and data consistency on heterogeneous storage. 
To achieve this, we combine transaction concurrency control and data persistence and redesign the data update method, using an Epoch-based logging method to ensure the consistency of heterogeneous storage.
Furthermore, an asynchronously logging method is adopted to optimize the transaction commit latency.

Building such a three-layer cloud-native database brings the following advantages:


\Paragraph{Empowering NoSQL DBs with Transaction Processing (TP) capability}
\label{Paragraph:Empowering NoSQL DBs with Transaction Processing (TP) capability}  
% NoSQL databases are popular because they store data in flexible schemas and can be scaled easily. Types of NoSQL databases include document databases \cite{mongodb, couchdbapache}, key-value stores \cite{hbase, leveldb, cassandra2014apache}, and graph databases \cite{wu2022nebula, neo4j}. However, 
Individual mutations (insert, update, and delete operations) in typical NoSQL DBs \cite{mongodb, couchdbapache, hbase, leveldb, cassandra2014apache, wu2022nebula, neo4j} are atomic and isolated at the row level.
Users can not group multiple operations accessing multiple rows into a transaction. 
Adding TP support for these systems requires an implementation effort to ensure the transaction's ACID properties, increasing development overhead. 
By sending transaction execution results (read and write sets) to TaaS for transaction management, NoSQL DBs can obtain TP capability.
TaaS maintains the meta-information of committed transactions to detect read-write and write-write conflicts between transactions to ensure atomicity, consistency, and isolation, and persists the logs locally to ensure durability.
As illustrative examples, we have empowered several NoSQL DBs, including LevelDB \cite{leveldb}, HBase \cite{hbase}, NebulaGraph \cite{wu2022nebula}, to support ACID transactions (Section \ref{subsection:Empowering NoSQL DBs with TP Capability}).


\Paragraph{Making Standalone TP Distributed} 
\label{Paragraph:Making Standalone TP Distributed}
Many standalone databases (\eg MySQL, PostgreSQL, and openGauss \cite{mysql, postgre, opengauss}) provide single-machine concurrent TP capability. However, their original versions do not support distributed TP and can not provide horizontal scalability. Extending standalone TP nodes to support distributed transactions is a complex task, requiring to carefully address concurrent conflicts in a distributed environment.
By connecting multiple identical standalone database instances to TaaS simultaneously, a multi-master distributed TP database system can be built. Each instance executes transactions independently and sends read and write sets to TaaS. 
TaaS resolves transaction concurrent conflicts and propagates the committed transactions' logs to all TaaS nodes for durability. It can achieve a certain degree of horizontal scalability by connecting a number of standalone database instances to TaaS.
For illustration, we construct a distributed TP database by connecting multiple openGauss \cite{opengauss} instances to TaaS (Section \ref{subsection:Making Standalone TP Distributed}).


\Paragraph{Supporting Cross-Model Transactions} 
\label{Paragraph:Supporting Cross-Model Transaction}
Modern business involves multiple data models (\eg relational, KV, graph, and vector) stored in various databases. %For example, a company may use a high-performance relational database to process financial-related business, a graph database to process relational networks, and a key-value database to store other data, such as images.
However, existing databases are typically designed to support a single data model. 
%Transactions involving multiple models must be split into multiple independent transactions, each involving only a single model. The commit or abort of all transactions needs to be consistent to ensure business correctness, which complicates the implementation of applications. Maintaining data consistency across the separate data stores is complicated.\zwx{added.}\zyf{don't know why you say the above two sentences.}
%zyf: you'd better just tell what you can do and why you do it in intro, but not how you do it. If you want discuss how, you should be very high-level. Refer to the above advantage
TaaS offers a solution for managing transactions that are processed by multiple execution engines with different data models (as shown in Figure \ref{fig:DB}). %We place a query proxy that distributes a client's operations to corresponding execution nodes. 
TaaS packages the execution results (read and write sets) from different execution nodes into a cross-model transaction to resolve transaction conflicts.
%, which access data cross data stores/models.
% By adding a storage identifier on records in the read and write sets \zyf{too detail, don't understand}, TaaS ensures the ACID attributes and the correctness of conflict resolution between cross-model transactions. 
As a result, we can support cross-model transactions by leveraging existing execution/storage engines with different data models, greatly reducing the development cost.
For illustration, we connect LevelDB \cite{leveldb} (KV store), openGauss \cite{opengauss} (relational DB), NebulaGraph \cite{wu2022nebula} (graph DB) to TaaS simultaneously to support cross-model transaction processing (Section \ref{subsection:Cross-Model Transaction}).

%\Paragraph{Achieving High Performance TP} 
%\label{Paragraph:Achieving high performance TP}
To maximize the performance and to ease of scaling, TaaS adopts a sharded multi-master architecture and employs a \textbf{\emph{Epoch-Based Sharded Multi-Master Optimistic Concurrency Control}} algorithm. By using an Epoch-Based Asynchronously Log Push-Down strategy, TaaS reduces the transaction latency. Notably, for read-intensive workloads where data updates are infrequent, this asynchronous strategy has little impact on performance due to reading stale data.
Our results show that by using the TaaS service, the system achieves 6.4 - 8.5 higher throughput and 4.9 - 5.8 times lower latency than these competitor systems on YCSB benchmark and 4.7 higher throughput and 5.1 times lower latency on TPC-C benchmark.

In summary, we make the following contributions: 
\begin{itemize}[leftmargin=*]
% \vspace{-0.05in}
    \item We propose a novel execution-transaction-storage three-layer cloud-native database architecture. The transaction management is decoupled from existing compute-storage disaggregated databases and works as an independent elastic service.
    % \vspace{-0.05in}
    \item We propose a multi-master optimistic conflict resolution mechanism that adapts to the servitization requirements of the transaction layer, which shows higher performance than existing disaggregated databases.
    % \vspace{-0.05in}
    \item We make several case studies of connecting existing execution/storage engines to TaaS to demonstrate the benefits of the three-layer architecture.
\end{itemize}

%The remainder of this paper is structured as follows: Section \ref{section:2} introduces related work. The workflow of the system will be introduced in Section \ref{section:3}. Section \ref{section:4} details the internal design and implementation of TaaS. Some case studies about TaaS are introduced in Section \ref{section:5}. In Section \ref{section:6}, we show experiments on TaaS. Some related work is in Section \ref{section:7}. In Section \ref{section:8}, we summarize the article and introduce some future work. 























%    ==========
%            ==
%            ==
%            ==
%    ==========
%            ==
%            ==
%            ==
%    ==========



By decoupling transaction management from the compute-storage disaggregated database system, an execution-transaction-storage three-layer cloud-native database architecture is constructed. In this section, we discuss the architecture and the overall execution workflow (Figure \ref{fig:overall_workflow}).



\subsection{Execution Layer}
\label{subsection:Execution Layer}
The execution layer consists of multiple stateless execution nodes (engines), which can be scaled up or down freely, achieving elasticity.
It is noticeable that there are multiple execution engines with different data models, such as KV, SQL, GraphQL (Graph Query Language), \etc. And we use the SQL execution as an illustration here.

After receiving a client's request, the parser transforms the statements (\eg SELECT) into parse trees, which are used to generate execution plans. The optimizer fetches metadata (\eg table schema and the distribution of data) from the storage layer through the \texttt{GetMeta} interface and generates physical execution plans. According to the physical execution plans, the operator then generates the read and write sets of transactions.
To increase concurrency and avoid blocking by locks, the execution layer adopts an \textit{optimistic} execution approach, where reads are obtained from the storage layer via the \texttt{GetData} interface without locking (\ie stale reads may exist) and writes are cached locally. 

Once a client commits a transaction, the cached read and write sets are sent to TaaS for transaction management through the \texttt{TxnCommit} interface.
After resolving transaction concurrent conflicts in TaaS, the transaction management result is returned to the execution node, and the execution node return the execution result with commit or abort to the client.
In order to interact with the TaaS layer, execution nodes need slight adjustments to adapt to the \texttt{TxnCommit} interface.



\subsection{Transaction Layer (TaaS)}
\label{subsection:Transaction Layer}

TaaS is designed as an independent transaction management service that ensures ACID properties of transactions. It is responsible for resolving transaction conflicts and provides a unified interface \texttt{TxnCommit} for the execution layer. To avoid any single TaaS node becoming a performance bottleneck, TaaS adopts a multi-master architecture, where multiple TaaS nodes can handle the read and write sets of transactions sent from the execution layer in parallel. This section gives a brief overview of how TaaS works. We will explain the detailed design of TaaS in Section \ref{section:4}.

Different workloads require different concurrency control algorithms. Prior work has proposed various concurrency control algorithms such as pessimistic two-phase locking \cite{yu2018sundial, lu2018star, harder1984observations}, optimistic \cite{yu2016tictoc, tu2013speedy, lu2021epoch, zhou2023geogauss}, and deterministic \cite{thomson2012calvin, lu2020aria, ren2019slog, qadah2020q} mechanisms, each with their own pros and cons. 
To build an independent service with scalability, availability, and elasticity, several requirements need to be considered. We will discuss these requirements in detail in Section \ref{subsection:Requirements}. Since there could be many choices that satisfy the requirements, we employ the \emph{\textbf{Epoch-Based Multi-Master OCC}} \cite{zhou2023geogauss} algorithm to resolve conflicts by default. 
% Note that TaaS also support other mechanisms \cite{} to resolve conflicts.

The concurrency control algorithm of TaaS takes the read and write sets of a transaction as input, and outputs the commit or abort decision of the transaction. 
After resolving transaction concurrent conflicts, the write sets of the transactions, which denote the updated data, are logged locally with the conflict resolution results that indicate the transaction commit or abort. Simultaneously, TaaS notifies the execution nodes of the results. 
To avoid synchronous waiting when updating the storage layer, TaaS leverages an active asynchronous log push-down method, where TaaS asynchronously propagates logs (\ie write sets of the committed transactions) to the storage layer through a \texttt{LogPush} interface.


% For each transaction, TaaS records its write set and decision before notifying the decision to the execution layer. TaaS also leverages an active asynchronous log push-down method, where TaaS asynchronously propagates logs (\ie write sets of the committed transactions) to the storage layer through a \texttt{LogPush} interface.

% % Effective transaction management depends heavily on the design of conflict resolution.
% One of key features \zyf{why features? the key of transaction management is...} in transaction management is transaction \zyf{write-write or read-write?} conflict resolution.
% Pessimistic two-phase locking \cite{yu2018sundial, lu2018star, harder1984observations}, optimistic \cite{yu2016tictoc, tu2013speedy, lu2021epoch, zhou2023geogauss}, and deterministic \cite{thomson2012calvin, lu2020aria, ren2019slog, qadah2020q} mechanisms adopted by previous works have their strengths and weaknesses, making them more suitable for specific scenarios \zyf{this sentence has grammar error. double check, which is subjective? what does each mean? each have?}. 
% As an independent service, several requirements need to be considered in building TaaS, which will be detailed \zyf{discussed in detail} in Section \ref{section:4}. Since there could be many choices that satisfy the requirements (Section 4.1), we choose an \emph{\textbf{Epoch-Based Multi-Master OCC}} \cite{zhou2023geogauss} algorithm to resolve transaction concurrent conflicts by default. 

% By adopting the epoch-based processing, TaaS nodes generate a snapshots at the completion of each epoch execution. TaaS achieves snapshot isolation level. 

% The workflow of TaaS can be described as follows: the read and write sets received from execution nodes over a period of time (epoch) is partitioned into a set on each TaaS node. After the previous epoch's execution is finished and a snapshot is generated, TaaS nodes uses the generated to validate the read sets and abort transactions, which execute incorrectly (\eg T3 in Figure \ref{fig:transaction conflict resolution}). Then, the write sets of transactions, which pass the read validation, are exchanged with every other TaaS node to ensure that each TaaS node updates the same data for each epoch. After receiving the write sets of the same epoch from all the other peer nodes, each TaaS node uses Algorithm \ref{alg:WriteSet Resolution} to resolve transaction concurrent conflicts independently. We will describe the conflict resolution in detail in Section \ref{subsection:Transaction Management}.

% After resolving transaction concurrent conflict, the transactions' write sets, which denote the updated data, are logged locally with the conflict resolution results that indicate the transaction commit or abort. Simultaneously, TaaS notifies the execution nodes of the results. 
% To avoid synchronous waiting when updating the storage layer, TaaS leverages an active asynchronous log push-down method.  After transactions are committed, TaaS asynchronously propagates the logs to the storage layer through a \texttt{LogPush} interface. 

% Additionally, TaaS provides a log-pulling interface for the storage, enabling the storage to pull missing logs caused by network fluctuation or machine failure. We will detail the logging mechanism in Section \ref{subsubsection:Logging}. 

% \pzs{TaaS is designed as an independent transaction management service to ensure transaction ACID properties. It is responsible for resolving transaction conflicts and provides a unified interface \texttt{TxnCommit} to connect different execution engines. TaaS consists of multiple servers. To prevent a single server from being a performance bottleneck, TaaS employs a multi-master architecture, where servers can perform the read set validation (in Section \ref{Paragraph:Read Set Validation}) and read-only transactions in parallel. We now briefly introduce the design of TaaS and its workflow before discussing in more detail in Section \ref{section:4}.}

% TaaS adopts an active asynchronously log push-down method to propagate the logs of committed transactions to the storage layer through a \texttt{LogPush()} interface by default. \pzs{this is not the reason to adopt asynchronously log push-down method.}
% Additionally, TaaS provides a log-pulling interface for the storage, enabling the storage to pull missing logs caused by network fluctuation or machine failure. We will detail the logging mechanism in Section \ref{subsubsection:Logging}. 

% The design of TaaS
% \pzs{Effective transaction management depends heavily on the design of conflict resolution. Pessimistic two-phase locking \cite{yu2018sundial, lu2018star, harder1984observations}, optimistic \cite{yu2016tictoc, tu2013speedy, lu2021epoch, zhou2023geogauss}, and deterministic \cite{thomson2012calvin, lu2020aria, ren2019slog, qadah2020q} mechanisms adopted by previous works each have their strengths and weaknesses, making them more suitable for specific scenarios. To meet the requirements as a independent service, TaaS adopts the \emph{\textbf{Epoch-Based Multi-Master OCC}} \cite{zhou2023geogauss} to resolve transaction conflicts.}

% % The workflow of TaaS
% \pzs{The workflow of TaaS can be described as follows: a TaaS server receives transactions from the execution layer and checks for transaction conflicts by validating their read sets. When an epoch ends, these transactions and their write sets are reliably broadcast to the other TaaS servers. These servers then independently resolve conflicts using these write sets and notify the execution layer of the results.}

% % logging
% \pzs{To avoid synchronous waiting when updating the storage layer, TaaS implements an active asynchronous log push-down method. After transactions are committed, each TaaS server stores their write sets as logs locally and asynchronously pushes them to the storage layer via the \texttt{LogPush} interface. In the event of network fluctuations or TaaS server failures, the storage layer also provides a log-pulling interface to retrieve missing logs. The logging mechanism will be further explained in Section \ref{subsubsection:Logging}.}

% TaaS consists of multiple TaaS servers and employs a multi-master architecture, where each TaaS server can handle the read and write sets received from the execution layer, to prevent a single TaaS server from being a performance bottleneck. This section briefly introduces the workflow of TaaS, and we will detail the design of TaaS in Section \ref{section:4}.   

% The key feature of transaction management is transaction conflict resolution. Previous works provide many design choices, such as pessimistic two-phase locking \cite{yu2018sundial, lu2018star, harder1984observations}, optimistic mechanisms \cite{yu2016tictoc, tu2013speedy, lu2021epoch, zhou2023geogauss}, and deterministic methods \cite{thomson2012calvin, lu2020aria, ren2019slog, qadah2020q}. Each algorithm has its own strengths and weaknesses, making them more suitable for certain scenarios. 
% As an independent service, several requirements need to be considered in building TaaS, which will be detailed in Section \ref{section:4}. To fetch these requirements, we choose an \emph{\textbf{Epoch-Based Multi-Master OCC}} \cite{zhou2023geogauss} algorithm by default.
% % Since only the read and write sets of a transaction are sent to the TaaS layer, the concurrency control of transaction management in TaaS becomes a read-write or write-write conflict resolution problem \zyf{why?}. Previous works provide many design choices for concurrency control, such as pessimistic two-phase locking \cite{yu2018sundial, lu2018star, harder1984observations}, optimistic mechanisms \cite{yu2016tictoc, tu2013speedy, lu2021epoch, zhou2023geogauss}, and deterministic methods \cite{thomson2012calvin, lu2020aria, ren2019slog, qadah2020q}. Each algorithm has its own strengths and weaknesses, making them more suitable for certain scenarios and we choose an \emph{\textbf{Epoch-Based Multi-Master OCC}} \cite{zhou2023geogauss} in TaaS \zyf{if you describe like this (using word choose), there is no contribution in transaction management, then why you need a section to discuss it?}. We will detail TaaS design later in Section \ref{section:4}. 
% After resolving transaction concurrent conflict, the transactions' write sets, which denote the updated data, are logged locally with the conflict resolution results that indicate the transaction commit or abort. Simultaneously, TaaS notifies the execution layer of the results. 

% TaaS adopts an active asynchronously log push-down method to propagate the logs of committed transactions to the storage layer through a \texttt{LogPush()} interface by default. \pzs{this is not the reason to adopt asynchronously log push-down method.}
% Additionally, TaaS provides a log-pulling interface for the storage, enabling the storage to pull missing logs caused by network fluctuation or machine failure. We will detail the logging mechanism in Section \ref{subsubsection:Logging}. 
% % \zyf{detail as a verb. is not commonly used. better: describe/present the logging mechanism in detail in Section...}


\subsection{Storage Layer}
\label{subsection:Storage Layer}

The storage layer consists of multiple storage nodes (\eg LevelDB \cite{leveldb}, HBase \cite{hbase}, MOT \cite{avni2020industrialmot}) that store data.
To provide the necessary metadata and the required data record for the execution layer, a storage adaptor is needed to be implemented to provide the \texttt{GetMeta} and \texttt{GetData} interfaces. Each storage node caches the frequently accessed data in its local in-memory buffer to reduce expensive disk IOs.
% \pzs{Better give a list of what the storage layer stores}
Since the data structure can be dramatically different between storage nodes, such as columnar storage \cite{abadi2008column}, row-column hybrid storage \cite{he2011rcfile}, graph-native storage \cite{deutsch2019tigergraph}, and vector storage \cite{wang2021milvus}, a logging adaptor should also be implemented by the developers to provide a specification on how to transform the TaaS committed logs to corresponding structured data. 

After finishing the transaction committing, TaaS begins asynchronous log pushing. For those storage nodes that provide updating interfaces, such as HBase \cite{hbase}, this logging adaptor can be implemented in the TaaS layer to minimize modifications to existing storage nodes. The adaptor transforms the logs to the corresponding structure, such as rowArray, rowOffset, rowLength \etc in HBase \cite{hbase}. Then, it invokes the interfaces (\eg \texttt{Put}) provided by HBase to update data. 
For the storage engines that do not offer a direct data update interface, such as the standalone databases like the openGauss \cite{opengauss}, modifications to the database are needed to implement the adaptor. After connecting to the TaaS and receiving the logs broadcast by TaaS, the adaptor fetches the table and row information and updates the row locally.

% To minimize modifications to existing storage servers,  is implemented in TaaS. \pzs{Q: how to covert read write set to different data structures?}
% When TaaS pushes logs to the storage layer, the adaptor invokes the data update interface provided by the storage layer to update data. For example, we implement a \textsf{Logger} in TaaS (Figure \ref{fig:transactionprocessing}), which invokes the \texttt{Put()} interface provided by HBase to update data.
% Suppose the storage engine the user selected does not offer a direct data update interface, such as the standalone databases like the openGauss \cite{opengauss}. In that case, modifications on the database are needed to connect to the TaaS Logger to receive and replay logs.

% The storage and logging adaptors should be correspondingly designed for different execution engines and storage engines. Take a graph query engine and graph-native storage as examples. The adaptor should provide a graph data query interface \zyf{why?} and update interface. 

% To minimize modifications to existing storage servers, this logging adaptor is considered to be implemented in TaaS first.
% When TaaS pushes logs to the storage layer, the adaptor invokes the data update interface provided by the storage layer to update data. For example, we implement a \textsf{Logger} in TaaS (Figure \ref{fig:transactionprocessing}), which invokes the \texttt{Put()} interface provided by HBase to update data.
% % This is because TaaS is designed as a pluggable service and can be independently upgraded, providing more agility than stateful storage servers. 
% Suppose the storage engine the user selected does not offer a direct data update interface, such as the stand-alone databases like the openGauss. In that case, modification are needed to connect to TaaS Logger, receive and replay logs to update data.

% The storage and logging adaptors should be correspondingly designed for different execution engines and storage engines. Take a graph query engine and graph-native storage as an example, the adaptor should provide a graph data query interface and graph data update interface. 












































































%    ==      ==
%    ==      ==
%    ==      ==
%    ==      ==
%    ==========
%            ==
%            ==
%            ==
%            ==




%\section{Coupled Transaction Processing and Data Replication}
\section{Transaction Layer Design}
\label{section:4}
\label{section:TaasLayerDesign}

In this section, we discuss the design and implementation of the transaction layer (TaaS), which ensures the transaction's ACID properties.

\subsection{Requirement Analysis}
\label{subsection:Requirements}

To achieve scalability, availability, and elasticity, TaaS must consider the following requirements.

First, TaaS should adopt a multi-master architecture.
The classic master-follower architecture adopted by cloud-native databases \cite{corbett2013spanner, huang2020tidb, taft2020cockroachdb, yang2022oceanbase} provides high availability but comes with several significant drawbacks. 
1) Distributed transactions are considered not scalable \cite{TheEndofaMyth, thomson2010casedeterminism, stonebraker2018onesizefitsall, ren2012lightweightlocking, kallman2008hstore, curino2010schism}. 
% Only one of the multiple replicas in a cluster can be a master node, which can resolve transaction concurrency conflicts. Increasing the number of replicas can not improve transaction management capacity. \pzs{Q: The first point and the second point are the same, i.e., transactions are not scalable because the master node resolves concurrency conflicts.}
Previous studies show that the database performance drops as the number of participant nodes increases on distributed transaction management \cite{zamanian2016end, mahmoud2014maat, salomie2011database}.
2) As all the conflict resolving requests must be sent to the master node, which causes heavy resource contention. The master node may be a single point of performance bottleneck in the system.
3) The master-follower architecture experiences temporarily unavailable when the master node goes down unexpectedly. The system necessitates a pause for complete log replaying in the followers.
% , so that the replica on the follower can be the same as the failed master's, ensuring correct conflicts resolution. \zyf{why you say this? master-follower ensures correct conflicts, so it is good?}

By adopting the multi-master architecture, each master node has the capability to receive and detect concurrent transaction conflicts. The read and write sets sent from execution nodes can be processed by any TaaS node. Since each TaaS node has a full replica of committed transactions' information, the read validation (Section \ref{Paragraph:Read Set Validation}) overhead can be distributed across all nodes. 
The transaction management capacity can be scaled by increasing the number of TaaS nodes. The transaction management capacity can be scaled.
As each TaaS node only needs to process a part of the transactions' read validation of the system, the single-node bottleneck can be avoided.
Each TaaS node can resolve transaction conflicts independently, thus, node failure can hardly affect the transaction management of other live nodes. 
As the workload changes, the cluster can scale up or down freely by adjusting the number of TaaS nodes, achieving elasticity.
% The cluster can scale-up or scale-down any master node freely to meets changing workloads.

% While the classic architecture adopted by cloud-native databases \cite{corbett2013spanner, huang2020tidb, taft2020cockroachdb, yang2022oceanbase}, popularized by System R* \cite{mohan1986r*},  adopts the sharded master-follower architecture to shard data on a set of shared-nothing machines horizontally \cite{eldeeb2023chardonnay} \zyf{don't understand. what's your point?}, it comes with several significant drawbacks. 
% 1)TP should be horizontally scalable with the increasing number of TaaS nodes. However, distributed transactions are considered not scalable \cite{zamanian2016end, mahmoud2014maat, salomie2011database}. The performance drops as the number of participant nodes increases, instead of taking advantage of the increasing computing capacity \zyf{no one speak English like this. instead of is misused.}. 
% 2) Only the master replica can handle the concurrency control, causing single server bottleneck. Furthermore, the system necessitates a pause for fault recovery procedures to ensure correct concurrency control, the system experiences temporary unavailability. \zyf{why you say single node bottleneck and availability together? they are not related. what's the relationship.}
% 3) A distributed commit protocol, such as the two-phase commit (2PC) \cite{mohan1985efficient2pc}, is needed to guarantee the atomicity of distributed transactions and a consensus protocol, e.g., Raft \cite{ongaro2014searchraft}, is used to back up transactions' logs and the 2PC state of committing transactions. 
% There are too many rounds of remote procedure calls (RPCs) in the system, causing high coordination overhead.
% % There are too many rounds of remote procedure calls (RPCs) to ensure the transactions ACID properties, .

% First, to function effectively \zyf{what is function effectively}, TaaS should adopt a multi-master architecture, wherein each TaaS server has the capability to receive and detect concurrent transaction conflicts. The read and write sets sent from different execution engines \zyf{should be execution instances. why you emphasize ``different''} can be processed by any TaaS server, distributing the read validate overhead across all servers and avoiding a single server bottleneck.
% Second, the 2PC is no longer necessitates \zyf{who defined 2PC is necessitates?} since every transaction is handled within a TaaS server \zyf{what's the logic?}. By introducing the Epoch-Based Commit protocol \cite{lu2021epoch}, the original transaction-level synchronization is transformed into epoch-level \zyf{logic error} %zyf: 你说因为我用了epoch-based commit protocol所以要用epoch-level sync，但是现在是要说你为什么用epoch commit，这个逻辑是混乱的
% , effectively reducing server coordination overhead. \zyf{why we have coordination overhead? do not assume reviewers know 2PC. you should use full name and briefly describe it.}
% Third, in the event of a server failure, the remaining servers only need to reach a consensus to exclude the failed machine from the cluster, and the system goes on execution \zyf{don't know why you should reach a consensus....}. Any TaaS server can be shut down, or a new node can join at any time; the service achieves high elasticity, scalability and availability. \zyf{comment}
%zyf: 你是想说这三个需求elasticity, scalability and availability， 对应三个design吗？如果是就明确在itemize的时候就解释，如果不是，我不懂为啥你这玩意就能达到这三个需求了。我觉得你这里是要重点motivate multi-master的design需求，multi-master可以达到elasticity, scalability and availability，对不？如果是，你往这上靠，multi-master方便随便加入离开，对应elasticity，还需要是coordinator-free的，这样可以有scalaility，multimater多副本还可以随便down，支持avaialiity

Second, epoch-based committing is more suitable in the multi-master architecture.
Since all TaaS nodes can resolve transaction conflicts, it is common to encounter conflicts between transactions from different TaaS nodes that read or update the same data item simultaneously. Multiple rounds of network communication are required to resolve such conflicts and achieve consensus for transaction submissions. It makes the coordination overhead heavy.
The Epoch-Based Commit protocol \cite{lu2021epoch} presents an approach to minimize communication overhead. By separating transactions into epochs and treating a whole epoch of transactions as the coordination unit, the original transaction-level synchronization is transformed into epoch-level, effectively reducing coordination overhead between nodes.

% 2) A distributed commit protocol is needed to guarantee the atomicity of distributed transactions when committing, such as the two-phase commit (2PC) \cite{mohan1985efficient2pc}. The coordinator in the 2PC uses two rounds \pzs{1.5 exactly.} of network communication to determine the commit status of participants in a distributed transaction, ensuring that the transaction is committed or aborted in all participants. To achieve failure recovery, a consensus protocol, e.g., Raft \cite{ongaro2014searchraft}, is used to back up transactions' logs and the 2PC state of committing transactions. Although some work \cite{guo2022cornus, gupta2018easycommit, al20041-2PC} propose optimizations on two-node commit protocols, there are still many rounds \pzs{How many rounds exactly.} of remote procedure calls (RPCs) in the system, causing high coordination overhead and reducing transaction management performance.

% Distributed commit protocols is no longer necessitates since every transaction commits within a TaaS server

% Third, the core of TaaS is transaction conflict resolution, ensuring multiple transactions can access and modify data concurrently without causing data inconsistencies. There are several concurrency control algorithms \cite{bernstein1987concurrency, yu2016tictoc, thomson2012calvin, wu2019anna}, each of which has its own strengths and weaknesses, making them more suitable for certain scenarios.

% For example, locking-based algorithms, such as two-phase locking, are commonly used in scenarios where data conflicts are likely to occur frequently and need to be resolved immediately. On the other hand, optimistic concurrency control algorithms, such as optimistic locking and validation-based protocols, are suitable for scenarios where conflicts are rare.
% Considering the requirements,  As all transactions' execution results are sent to the transaction layer for management, it is natural to choose OCC \cite{occ} which detects conflicts during committing. \zyf{the logic is not clear}

% Third, the core of TaaS is transaction conflict resolution, ensuring multiple transactions can access and modify data concurrently without causing data inconsistencies. 
% There are several concurrency control algorithms \cite{bernstein1987concurrency, yu2016tictoc, thomson2012calvin, wu2019anna}, each of which has its own strengths and weaknesses, making them more suitable for certain scenarios.
% % For example, locking-based algorithms, such as two-phase locking, are commonly used in scenarios where data conflicts are likely to occur frequently and need to be resolved immediately. On the other hand, optimistic concurrency control algorithms, such as optimistic locking and validation-based protocols, are suitable for scenarios where conflicts are rare.
% Considering the requirements, the concurrent control algorithm used in TaaS should follow the multi-master architecture. As all transactions' execution results are sent to the transaction layer for management, it is natural to choose OCC \cite{occ} which detects conflicts during committing. \zyf{the logic is not clear}

\begin{figure}
     % \begin{minipage}{0.5\textwidth}
        % \centerline{\includegraphics[height=2in]{figs/taas_flow_example auto crop.pdf}}
        \centerline{\includegraphics[height=2in]{figs/taas_flow_example flow auto crop.pdf}}
        \centering
        \vspace{-0.13in}
        \caption{Transaction processing in TaaS.}
        \vspace{-0.1in}
        \label{fig:transactionprocessing}
    % \end{minipage}
\end{figure}


% \begin{figure*}
%     \begin{minipage}{0.5\textwidth}
%         % \centerline{\includegraphics[height=2in]{figs/taas_flow_example auto crop.pdf}}
%         \centerline{\includegraphics[height=2in]{figs/taas_flow_example flow auto crop.pdf}}
%         \centering
%         \vspace{-0.1in}
%         \caption{Transaction processing in TaaS.}
%         \vspace{-0.1in}
%         \label{fig:transactionprocessing}
%     \end{minipage}
%     \begin{minipage}{0.49\textwidth}
%         \centerline{\includegraphics[height=2in]{figs/epoch_validate_blob_autocrop.pdf}}
%         \centering
%         \vspace{-0.1in}
%         \caption{Transaction conflict resolution in TaaS.}
%         \vspace{-0.1in}
%         \label{fig:ReadSetValidation}
%     \end{minipage}
% \end{figure*}


\subsection{Transaction Management}
\label{subsection:Transaction Management}

In this subsection, we first describe the TaaS-side transaction processing, conflict resolution, and logging.




\subsubsection{Transaction Processing} 
The core of TaaS is transaction conflict resolution, ensuring multiple transactions can access and modify data concurrently without breaking the transaction ACID properties.
The concurrency control algorithm of TaaS has multiple choices \cite{thomson2012calvin, zhou2021foundationdb, wu2019anna, lu2020aria, zhou2023geogauss} to satisfy the requirements listed in Section \ref{subsection:Requirements}.
Inspired by GeoGauss \cite{zhou2023geogauss}, we propose an \emph{\textbf{Epoch-Based Multi-Master Optimistic Concurrency Control}} algorithm to resolve transaction conflict by default.
By adopting such epoch-based processing, TaaS nodes generate a snapshot at the completion of each epoch execution so that it can achieve the snapshot isolation level. 

As illustrated in Figure \ref{fig:transactionprocessing}, the \textsf{Client Proxy} provides the \texttt{TxnCommit} service interface for the execution nodes. When receiving a transaction management request along with its read and write sets from an execution node, the \textsf{Client Proxy} tags the related commit-info for the current transaction, which will used in the subsequent transaction conflict resolution:

\begin{itemize}[leftmargin=*]
    \item Commit Epoch Number (cen) is used to distinguish which epoch the transaction belongs to. TaaS divides physical time into epochs (e.g., 10ms per epoch) and assigns incremental unique numbers to these epochs. TaaS packages transactions received over a period of time (epoch) into a set and processes transaction management at epoch granularity.

    \item Commit Sequence Number (csn) is used to determine transaction order within an epoch. Unlike TiDB \cite{huang2020tidb} or FoundationDB \cite{zhou2021foundationdb}, which use a global timestamp ordering service, the csn is \textit{globally unique}, which is generated based on a local timestamp and a local TaaS node ID (integer). It is assigned locally by each TaaS node to avoid a single time node's bottleneck. We use a comparison method to determine transactions partial order `$\prec$' based on the csn: 1) transaction with an older local time $\prec$ transaction with an older local time. 2) transaction with a smaller node id $\prec$ transaction with a bigger node id when transactions have the same local time. Transaction with the smaller csn wins in the conflict resolution. \textcolor{blue}{Choosing a lower CSN does make it easier for transactions to win in conflicts. Transactions accepted by the TaaS node with lower csn assignment are more likely to commit, with partial unfairness. It is worth stating that the comparison rules within epoch are changeable, for example, the comparison rule can be based on CSNs and server node numbers, and that TaaS handles transactions a bit more fairly.}
\end{itemize}

The \textsf{Epoch Manager} is responsible for monitoring the process of epoch transaction conflict management, ensuring advancing epoch correctly.
After the set of transactions (read and write sets) of the previous epoch have been executed and a snapshot is generated, it notifies the \textsf{Client Proxy} to start the \textbf{Read Set Validation} of local current epoch transactions to ensure data consistency. We will describe more details in Section \ref{Paragraph:Read Set Validation}.

Then, the \textsf{Client Proxy} transports the transactions that pass the read set validation phase to the \textsf{Message Transporter} to propagate the write sets to other nodes. 
To ensure the replica consistency between TaaS nodes and the correctness of transaction management according to \cite{zhou2023geogauss}, each TaaS node must synchronize the epoch transactions' write sets with other nodes so that all TaaS nodes process the same write sets of the current epoch. 
% According to \cite{zhou2023geogauss}, each TaaS node must synchronize the epoch transactions' write sets with other nodes so that all TaaS nodes process the same write sets of the current epoch, ensuring the replica consistency between TaaS nodes and the correctness of transaction management. 



After completing sending the local transaction set and receiving the transaction sets (write sets) of the same epoch from all the other peer nodes, the \textsf{Epoch Manager} notifies the \textsf{Client Proxy} sends the local transaction set to the \textsf{Conflict Resolver}, which uses the Write Set conflict Resolution Algorithm (Algorithm \ref{alg:Write Resolution}) to resolve write-write conflicts between transaction within the epoch (\textbf{Write Set Resolution}). The remote node transaction sets will also be sent to the \textsf{Conflict Resolver} so that all TaaS nodes process the same set of transactions, ensuring the conflict resolution results of an epoch are the same.

After conflict resolution, the resolution results that indicate the successful updates are logged on the local disk and returned to execution nodes. The committed logs will be lazily sent to the storage layer by the \textsf{Logger}.








\subsubsection{Transaction Conflict Resolution}
\label{subsubsection:Transaction Conflict Resolution}

There exist two types of conflicts in TaaS: A read-write conflict that occurs when a transaction T1 updates a value that has been read by an uncommitted transaction T2, and a write-write conflict that occurs when the value written by T1 is overwritten by T2. TaaS resolves read-write conflicts with the read set validation, while write-write conflicts are resolved with the write set conflict resolution algorithm.

\begin{figure}[t]
     % \begin{minipage}{0.5\textwidth}
        % \centerline{\includegraphics[height=2in]{figs/taas_flow_example auto crop.pdf}}
        \centerline{\includegraphics[height=2in]{figs/epoch_validate_blob_autocrop.pdf}}
        \centering
        \vspace{-0.1in}
        \caption{Transaction conflict resolution in TaaS.}
        \vspace{-0.1in}
        \label{fig:transaction conflict resolution}
    % \end{minipage}
\end{figure}

\Paragraph{Read Set Validation}
\label{Paragraph:Read Set Validation}
As shown in Figure \ref{fig:transaction conflict resolution}, a read-write conflict occurs when T1 updates X, which has already been read by T3. Specifically, the initial values of X, Y, and Z are all 1. T1 first updates both X and Y to 5 and commits them successfully on TaaS. Due to the asynchronous update of the storage layer, the subsequent transaction T3 reads X with the latest value 5 while Y with the stale value 1. Although T3 has no conflicts with transactions within the same epoch, it must still be aborted to ensure transaction atomicity (\ie T3 should read all the values updated by T1 or none of them). 
The read set validation is to ensure the atomicity, consistency and isolation of transactions.
% To ensure transaction atomicity, consistency and isolation, the read set validation is needed.
By using snapshots generated at the end of each epoch's execution, the \textsf{client proxy} aborts transactions break the atomicity (\eg the value of Y in T3's read set is not equal to TaaS's snapshot).
% As all the meta-information of committed transactions is stored on TaaS servers, the update granularity of the storage node does not affect TaaS transaction management.  \pzs{What for?} % 不要提存储层吧，这里在讲事务处理


% \begin{algorithm}[t]
% \begin{spacing}{1}
% \SetAlgoNoLine
% \small
%     \caption{Write Set Resolution Algorithm (Update and Delete)}
%     \label{alg:WriteSet Resolution}
%     \KwIn{a transaction in TaaS $txn.\{csn, WS\}$, 
%     GlobalWriteVersionMap stores committed transactions' modifications ,
%     EpochWriteVersionMap detects write-write conflict between transactions of current epoch, 
%     and EpochAbortSet stores the csn of transactions, which should be aborted in current epoch.}
%     \KwOut{return commit or abort}
%     \SetKw{Continue}{continue}
    
%      $result = true$\;
%     \ForEach{$record$ \rm{in} $txn.WS$}{
%         $row$ = GlobalWriteVersionMap.Find($record$.key)\;
%         \uIf{$row == NULL$}{
%             $result = false$; \textcolor{gray}{ \hspace{0.1in} //deleted by a previous epoch txn.}\\
%             \Continue\;
%         }
%         $row$ = EpochWriteVersionMap.Find($record$.key)\;
%         \uIf{$row == NULL$}{
%            \textcolor{gray}{ //row has not been updated in current epoch.}\\
%             $row.\{csn\} = txn.\{csn\}$\;
%             EpochWriteVersionMap.Set($row$)\;
%         }
%         \uElseIf{($row.csn > txn.csn$)} {
%             \textcolor{gray}{ //write-write conflict within the epoch, based on the partial order '$\prec$', current txn wins.}\\
%             EpochAbortSet.Insert($row.csn$)\;
%             $row.\{csn\} = txn.\{csn\}$\;
%             EpochWriteVersionMap.Set($row$)\;
%         }
%         \uElse{
%             $result = false$\;
%         }
%     }
%     \uIf{$result == false$} {
%         EpochAbortSet.Insert($txn.csn$)\;
%     }
%     \KwRet $result$\;

    
% \end{spacing}
% \end{algorithm}

\begin{algorithm}[t]
\begin{spacing}{1}
\SetAlgoNoLine
\small
    \caption{Write Set Conflict Resolution}
    \label{alg:Write Resolution}
    % \KwIn{a transaction in TaaS $txn.\{csn, WS\}$, 
    % GlobalWriteVersionMap stores committed transactions' information ,
    % EpochWriteVersionMap detects conflicts between transactions of current epoch, 
    % and EpochAbortSet stores the csn of transactions, which should be aborted in current epoch.
    \KwIn{a transaction in TaaS $txn.\{csn, WS\}$.}
    \KwOut{Commit or Abort}
    \SetKw{Continue}{continue}

    \SetKwFunction{FWriteSetResolution}{WriteSetResolution}
    \SetKwFunction{FCompare}{Compare}

    \SetKwProg{Fn}{Function}{:}{\KwRet}
    \Fn{\FWriteSetResolution{Transaction $txn$}}{
        $result = Commit$\;
        \ForEach{$r$ in $txn.WS$}{
            $row$ = GlobalWriteVersionMap.Find($r$.key)\;
            \uIf{$row$ is not $Null$ \textbf{and} $r.type$ is $Insert$}{
                    $result = Abort$; \textcolor{gray}{//rwo already exists.}\\
            }
            \uElseIf{$row$ is $Null$ \textbf{and} $r.type$ is not $Insert$}{
                    $result = Abort$; \textcolor{gray}{ //deleted in previous epoch.}\\
            }
            \uElse{
                $result$ = Compare($r$)\;
            }
        }
        \uIf{$result$ is $Abort$} {
            EpochAbortSet.Insert($txn.csn$)\;
        }
        \KwRet $result$\;
    }

    \SetKwProg{Fn}{Function}{:}{\KwRet}
    \Fn{\FCompare{Record $r$}}{
        $row$ = EpochWriteVersionMap.Find($r$.key)\;
        \uIf{$row$ is $Null$}{
           \textcolor{gray}{ //row has not been updated in current epoch.}\\
            $row.csn = txn.csn$\;
            EpochWriteVersionMap.Set($row$)\;
        }
        \uElseIf{($row.csn > txn.csn$)} {
                \textcolor{gray}{ //mark the transaction with csn $row.csn$ as abort.}\\
                EpochAbortSet.Insert($row.csn$)\;
                $row.csn = txn.csn$\;
                EpochWriteVersionMap.Set($row$)\;
            }
            \uElse{
                \KwRet $Abort$\;
            }
        % }
        \KwRet $Commit$\;
    }
\end{spacing}
\end{algorithm}

\Paragraph{Write Set Conflict Resolution}
\label{Paragraph:Conflict Resolution}
TaaS leverages a write set conflict resolution algorithm (Algorithm \ref{alg:Write Resolution}) to resolve write-write conflicts of concurrent transactions within the same epoch. TaaS uses the primary key of a data item to detect transaction conflicts. For data items without an explicit primary key, an implicit primary key needs to be used and transferred to TaaS for conflict handling. Each TaaS node uses a \textit{GlobalWriteVersionMap} to store the committed transaction's information on data items, an \textit{EpochWriteVersionMap} for modification intent to detect write-write conflicts between transactions in the same epoch, and a \textit{EpochAbortSet} to store the csn of which should be aborted in the current epoch.

When performing the write set resolution of a transaction, the \textsf{Conflict Resolver} invokes the \texttt{WriteSetResolution} function and traverses each record (\eg row) in the transaction's write set to detect whether a conflict exits with other transactions. 
The \textsf{Conflict Resolver} searches for the row's state from the \textit{GlobalWriteVersionMap} with the primary key of the data item first and processes different judgments depending on the existence of the row and the type of the operation in the write set:
1) The row is not null and the operation type of the record is Insert means that the row that the current transaction wants to insert has already been inserted by another transaction that has been committed. This behavior is prohibited, and the \textsf{Conflict Resolver} aborts the transaction (lines 5-6).
2) The row is null and the operation type of the record is Update/Delete means that the row does not exist or has been deleted in the previous epoch. The transaction should also be aborted (lines 7-8).
3) In other cases, the operation that the transaction wants to perform is allowed. Then, the \textsf{Conflict Resolver} uses the \texttt{Compare} function to detect conflicts within the epoch (lines 9-10).

In the \texttt{Compare} function, the \textsf{Conflict Resolver} searches the \textit{EpochWriteVersionMap} to detect whether there is a transaction has tried to update this row since the beginning of the write set conflict resolution.
: 1) $row == NULL$ means that there is no other transaction trying to update this row, the \textsf{Conflict Resolver} marks the row with the current transaction's csn, representing that the transaction is allowed to update the rows at the current epoch temporarily (lines 16-19).
2) Otherwise, there is a transaction that already updates this row and a write-write conflict occurs in the current epoch. We use the partial order, `$\prec$', to determine that a transaction with a smaller timestamp can update the row (lines 20-26). 
It is worth noticing that by using the local clock with TaaS node ID to assign csn, no two transactions with the same csn exist in TaaS, so the case of $row.csn == txn.csn$ will never occur.

After completing the conflict resolution of all transactions, the \textsf{Conflict Resolver} aborts the transactions according to the \textit{EpochAbortSet}, updates the \textit{GlobalWriteVersionMap}, and writes logs locally. Then, a new snapshot based on the current epoch is generated.
It is important to highlight that TaaS stores only metadata (\eg record key, csn) for concurrency control in memory without retaining the entire data set. As a result, TaaS incurs minimal memory overhead.

By using the \texttt{Compare} function, which equips commutative by using the partial order `$\prec$', the conflict-resolution results of each TaaS node with the same epoch are the same even with a different transaction processing order. 
TaaS nodes can maximize the parallel resolution of conflicts and ensure the correct transaction management and replica consistency.
More detailed proof of the commutative and correctness are represented in \cite{zhou2023geogauss}.


\Paragraph{CC Variation-Sharding}
\label{Paragraph:CC Variation}
Under the multi-master architecture, each TaaS node can independently validate the transaction's read set, providing high read scalability. The system works well under read intensive workloads. However, all writes are needed to be processed on every TaaS node to ensure the consistency (write amplification). 

To achieve scalability under write intensive workloads, we implement an epoch-based sharding variation on TaaS. By adopting a sharding strategy (\eg hash), TaaS split data into multiple shards and each TaaS node is responsible for a set of disjoint shards. After receiving a transaction from the execution layer, the TaaS node shards the transaction into multiple sub-transactions (sharded read and write set) with the same cen and csn and sends these sub-transactions to the corresponding TaaS nodes. Once the TaaS node completes receiving all sub-transactions of the current epoch, it does the \textbf{Read Set Validation} and \textbf{Write Set Resolution} for these sub-transactions. Then, TaaS nodes exchange local \textit{EpochAbortSet} with others and merge all \textit{EpochAbortSets} into a global one. Finally, TaaS nodes abort transactions based on this global \textit{EpochAbortSets}. In the sharding variation, an additional synchronization is needed for TaaS nodes to collect the all\textit{EpochAbortSet} of the entire cluster. This is because that sub-transaaction wins in local conflict resolution may lose on another node, TaaS nodes need to notify sub-transaction conflict results with each other so that transactions across multiple TaaS nodes can be committed or aborted atomically. 




\subsubsection{Isolation}
\label{Paragraph:Isolation}
By using an epoch-based resolution mechanism, TaaS supports snapshot isolation level by default. 
TaaS also support Read Committed (RC) and Repeatable Read (RR) isolation levels only when the storage layer supports transaction-granularity data updates, as the storage layer that only supports row level isolation cannot guarantee the correctness of transaction (\eg T3 in Figure \ref{fig:transactionprocessing}).
% TaaS can support RC by skipping the \textbf{Read Set Validation}, and support RR by checking transaction's own read set.
TaaS does not support SSI isolation level when adopting the epoch-based OCC algorithm, since transactions' read sets and write sets are needed to be transported between multiple TaaS nodes to detect read-write dependency within the epoch, which causes much higher network transmitting overhead. 
As a result, TaaS has chosen to discard this isolation level for the time being. We discuss the possible implementations of this isolation level here. One option is to build a read-write dependency graph and break the dependency loop \cite{serializablesnapshotisolation}. 



\subsubsection{Logging}
\label{subsubsection:Logging}
TaaS implements a lightweight logging method to store logs locally without the support of the storage layer. Concurrently, it initiates an active asynchronous log push-down strategy to minimize transaction latency.

To prevent performance bottlenecks when pushing logs, each TaaS node only transmits committed transactions' logs received by itself. 
Nevertheless, when utilizing the asynchronous method, the pushing-down epoch on each node may differ. Transactions across epochs may encounter write-write conflicts. When different TaaS nodes are pushing logs for different epochs via the interface provided by the storage nodes (\eg \texttt{Put}), update conflicts may occur. So, a synchronization between TaaS nodes is needed to ensure that logs are pushed down correctly.
For those distributed storage nodes (\eg HBase \cite{hbase}, TiKV \cite{tikv}), each TaaS node invokes the log adaptor implemented within TaaS to push epoch logs.
For those storage nodes that do not provide a unified interface, the implemented adaptor needs to connect to all TaaS nodes to collect a complete log set. After completing the collection, the adaptor replays the logs in epoch order. 
% \pzs{see comments, must discuss the workflow of the adaptor to standalone db or storage service.}
% % 需要详细讲一下存储层单机系统怎么做的分布式，就是PUT的具体实现流程（也可以说是adaptor的实现流程）

% TaaS implements various log update methods to accommodate different storage nodes. 
% For storage nodes that offer a data update interface, such as HBase, the \textsf{Logger} invokes the interfaces to replay logs. 
% For storage nodes lacking such interfaces, like the stand-alone database openGauss, slight modifications are required to be made on the storage servers to connect the logging adaptor to receive and replay logs. 

% \pzs{What is this paragraph for? I cannot follow it.}
% In the multi-master architecture, each TaaS server maintains a complete copy of these logs. To prevent performance bottlenecks, each server only transmits local transaction logs. 
% Nevertheless, when utilizing the asynchronous method, the pushing-down epoch on each server may differ, causing update conflicts between transactions belonging to different epochs.
% So, a synchronize is placed when log pushing, ensuring that logs are pushed down in the sequence of epochs.
% In essence, transaction conflict resolution and log push-down are carried out asynchronously, while the progress of epoch log push-down between servers is synchronized. The data in the storage layer is updated at the epoch granular.

% Additionally, TaaS provides a \texttt{LogPull} interface to pull specific logs for system recovery. 

% \pzs{Q: TaaS service is multi-mastered, meaning it has multiple replicas processing the same set of transactions and generating the same batch of logs. However, the storage service count may be different from TaaS replica count. So how does TaaS replica push down its log to the storage?}

% In the multi-master architecture, each TaaS server maintains a complete copy of these logs. Storage nodes connect to a TaaS server randomly to receive logs.
% When utilizing the asynchronous method, the pushing-down epoch on each server may differ. To ensure that 
% Meanwhile, TaaS servers periodically perform garbage collection of the epoch logs that have been pushed down successfully to avoid a large amount of storage overhead.








% \subsubsection{Consistency}
% \label{subsubsection:Consistency}

% Now, we discuss the consistency of replicas and there are a few principles in TaaS.
% 1) By using the monotonically of the Epoch, the \textsf{Epoch Manager} ensures that the next epoch transaction can not start until the execution of the previous one is completed. Each TaaS server generates snapshots in sequence. 
% 2) Data consistency is ensured by processing the read set validation based on the snapshots. 3) Each replica instance can get the same output (\textit{EpochAbortSet}) with the same input (the complete epoch transaction sets) by using Algorithm \ref{alg:Conflict Handling} which equips commutative by using the partial order '$\prec$'. TaaS servers do not need to consider the transactions' execution order within the same epoch.

% Since the initialize of each replica is the same. The updates of each epoch are the same among TaaS servers (3) and do not break data consistency (2). Each TaaS server uses the same output to update the replica in order (1), generating same snapshots at the end of each epoch. Therefore, each replica in the transaction layer guarantees consistency at epoch granularity.


% \begin{lemma}
% \label{lemma:readvalidate}
% Data consistency is ensured by processing the read set validation.
% \end{lemma}
% \textbf{Proof.} Each Taas server generates snapshots at the epoch basis and uses these snapshots to perform read set detection on transactions in the next epoch. TaaS aborts the transactions with error execution results(Figure \ref{fig:ReadSetValidation}, T3) to prevent data inconsistency.
% % \zwx{consistency between TaaS and the storage layer}
% %由于所有已提交的事务元信息都保存在TaaS端，不同存储引擎之间的数据短暂不一致不会影响TaaS的事务管理。因为TaaS的读集验证能够保证数据一致性。

% \begin{lemma}
% \label{lemma:determinewrite}
% The committed transaction sets that each server generated at the same epoch are the same.
% \end{lemma}
% \textbf{Proof.} 
% The transaction conflicts within an epoch are handled by using Algorithm \ref{alg:Conflict Handling} which equips commutative by using the partial order '$\prec$'. TaaS servers do not need to consider the transactions' execution order within the same epoch. Multiple replica instances can get the same output of the abort set with the same input (the complete epoch transaction sets). Meanwhile, TaaS servers commit or abort transactions based on the same \texttt{EpochAbortSet}. 
% Thus, the conflict-handling results of each replica with the same epoch are the same.

% \begin{lemma}
% \label{lemma:monotonicity}
% The snapshot of epochs in each server are monotonically increasing.
% \end{lemma}
% \textbf{Proof.} Using the monotonically of the Epoch, the \textsf{Epoch Manager} ensures that the next epoch transaction can not start until the execution of the previous one is completed. Each TaaS server generates snapshots in sequence.

% \begin{theorem}
% \label{theorem:consistencyreplicas}
% The replicas in transaction layer are consistent at the granularity of epochs.
% \end{theorem}
% \textbf{Proof.} Since the initialize of each replica is the same. The updates of each epoch do not break data consistency (\textit{\textbf{Lemma \ref{lemma:readvalidate}}}) and are the same among TaaS servers (\textit{\textbf{Lemma \ref{lemma:determinewrite}}}). Each TaaS server uses the same output to update the replica in order (\textit{\textbf{Lemma \ref{lemma:monotonicity}}}), generating the globally consistent snapshot.
% Therefore, each replica in the transaction layer guarantees consistency at epoch granularity.








\subsection{Fault Recovery}
\label{subsection:Fault Recovery}

In the execution-transaction-storage architecture, since all execution nodes are stateless, we focus on the recovery of TaaS and the storage layer.

% The failure of an execution server does not disrupt the transaction or storage layer. In the event of an executor failure, the system simply restarts the executor and resumes processing new user requests. Transactions submitted to TaaS will not be affected; the conflict handling and the data updating will proceed as usual. However, users may lose transaction submission results as they have disconnected from the execution engine.

TaaS adopts the Raft \cite{ongaro2014searchraft} protocol to tolerate the failures of no more than half of the TaaS nodes. Every TaaS node reliably replicates its transactions to others via its own Raft instance. As each node maintains a full copy of the meta-information of committed transactions, unexpected TaaS node failures will not affect the availability of TaaS. Moreover, execution nodes connected to the failed TaaS nodes are routed to other healthy TaaS nodes, ensuring uninterrupted transaction management service.
When TaaS nodes fail, other TaaS nodes will be notified by a timeout because TaaS nodes use the Raft consensus to ensure the atomic broadcast of their transactions. To avoid blocking after a node failed, another TaaS node is elected as the Raft leader to replace the failed node. The leader pushes down the logs the failed node should do to keep the storage layer updated. Even when the majority of TaaS nodes fail due to network partitions or power outages, TaaS can still provide read-only service. When a TaaS node recovers from failures, it first pushes down its local remaining logs (no TaaS node can be selected as the leader in this situation). Since all its memory states are lost, it then catches up with the latest state by fetching the Raft logs from other TaaS nodes before providing service.

As described in Section \ref{subsection:Storage Layer}, the storage layer may consist of distributed storage services like TiKV \cite{tikv} and standalone databases like openGauss \cite{opengauss}. Since distributed storage services already provide fault tolerance, the storage layer does not need to perform any additional fault tolerance mechanisms for them. When building the storage layer with standalone databases, deploying multiple standalone instances (nodes) is needed. Since each instance has a full copy of the data, the majority of storage nodes failed can not effect the storage layer providing data service. When a node recovers, it pulls logs from TaaS during the recovery phase by invoking the \texttt{LogPull} interface supported by TaaS and replays the logs. 


% TaaS adopts a multi-master architecture, and each node maintains a full replica of the meta-information of committed transactions and uses the Raft \cite{ongaro2014searchraft} protocol to transmit the transaction sets. When a TaaS node goes down, other nodes can promptly take over the role of the failed node, ensuring uninterrupted transaction management service for users.
% In addition, TaaS employs an additional Raft protocol consensus group to monitor the cluster's status, preventing extended blocking (each node must collect the complete transaction set of an epoch) in case of node failure. If a node fails, the Raft leader takes over the duties of the failed node, transmitting unpushed logs to the storage layer from the period of downtime to the point of consensus achieved. During the node's recovery phase, the node pulls meta-information from other TaaS nodes and re-joins the TaaS cluster.
% % Since TaaS employs an approach in which each server is responsible for asynchronous push-down of a part of the epoch logs (Section \ref{subsec:Logging}), 
% If TaaS fails, the system can still provide read-only service. When TaaS returns back to the system, TaaS first pushed the unfinished logs to the storage layer and starts to provide service. Since all the committed transactions' meta-information that is stored in memory is lost, TaaS will abort the read-write transactions that start before the recovery.

% The recovery process for TaaS server failures closely resembles the recovery process of the storage engine in a multi-master expansion. During recovery, the server must reinstate meta-information to ensure the accurate handling of concurrency conflicts.
% In TaaS, the \textit{WriteVersionMap} and the \textit{ReadVersionMap} are consistent after each epoch finished. Consequently, the TaaS server only needs to request the most recent version of the \textit{ReadVersionMap} from other replicas. Subsequently, the TaaS server replays the logs to update the \textit{ReadVersionMap} to the latest version, re-joins the TaaS cluster, and resumes receiving transaction processing requests.
 
% For using TaaS to expand from a stand-alone database to a multi-master architecture, the failure of a single instance does not affect the entire cluster because each instance has a full copy of data. The remaining instances can still provide service.
% When the failed instance recovers and rejoins the cluster, it pulls logs from TaaS during the recovery phase by invoking the \texttt{LogPull} interface supported by TaaS. If TaaS has performed garbage collection on the logs, the node needs to pull a recent database snapshot from other replicas and replays the recent logs to update the data to the latest version. 
% Once the storage layer goes down, the system can no longer provide data access service. By employing a heartbeat mechanism, TaaS detects the aliveness of the storage layer and stops the log pushing until the storage layer returns to the system.


==> sigmod.tex <==
% %%
% %% This is file `sample-sigconf.tex',
% %% generated with the docstrip utility.
% %%
% %% The original source files were:
% %%
% %% samples.dtx  (with options: `sigconf')
% %% 
% %% IMPORTANT NOTICE:
% %% 
% %% For the copyright see the source file.
% %% 
% %% Any modified versions of this file must be renamed
% %% with new filenames distinct from sample-sigconf.tex.
% %% 
% %% For distribution of the original source see the terms
% %% for copying and modification in the file samples.dtx.
% %% 
% %% This generated file may be distributed as long as the
% %% original source files, as listed above, are part of the
% %% same distribution. (The sources need not necessarily be
% %% in the same archive or directory.)
% %%
% %% Commands for TeXCount
% %TC:macro \cite [option:text,text]
% %TC:macro \citep [option:text,text]
% %TC:macro \citet [option:text,text]
% %TC:envir table 0 1
% %TC:envir table* 0 1
% %TC:envir tabular [ignore] word
% %TC:envir displaymath 0 word
% %TC:envir math 0 word
% %TC:envir comment 0 0
% %%
% %%
% %% The first command in your LaTeX source must be the \documentclass command.
% \documentclass[sigconf, nonacm]{acmart}
% %% NOTE that a single column version is required for 
% %% submission and peer review. This can be done by changing
% %% the \doucmentclass[...]{acmart} in this template to 
% %% \documentclass[manuscript,screen]{acmart}
% %% 
% %% To ensure 100% compatibility, please check the white list of
% %% approved LaTeX packages to be used with the Master Article Template at
% %% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
% %% before creating your document. The white list page provides 
% %% information on how to submit additional LaTeX packages for 
% %% review and adoption.
% %% Fonts used in the template cannot be substituted; margin 
% %% adjustments are not allowed.

% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

% %% Rights management information.  This information is sent to you
% %% when you complete the rights form.  These commands have SAMPLE
% %% values in them; it is your responsibility as an author to replace
% %% the commands and values with those provided to you when you
% %% complete the rights form.
% \setcopyright{acmlicensed}
% \copyrightyear{2024}
% \acmYear{2024}
% \acmDOI{XXXXXXX.XXXXXXX}

% %% These commands are for a PROCEEDINGS abstract or paper.
% % \acmConference[Conference acronym 'XX]{Make sure to enter the correct
% %   conference title from your rights confirmation emai}{June 03--05,
% %   2018}{Woodstock, NY}
% %
% %  Uncomment \acmBooktitle if th title of the proceedings is different
% %  from ``Proceedings of ...''!
% %
% %\acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
% %  June 03--05, 2018, Woodstock, NY} 
% % \acmISBN{978-1-4503-XXXX-X/18/06}

% \usepackage{enumerate}
% \usepackage[linesnumbered, ruled, vlined, noend, resetcount]{algorithm2e} % For Algorithm
% \usepackage{graphics}
% \usepackage{balance}
% \usepackage{graphicx}
% \usepackage{subfig}
% \usepackage{amsthm}
% \usepackage{bm}
% \usepackage{algpseudocode}
% \usepackage{listings}
% \usepackage{enumitem}
% \usepackage{multirow}
% \usepackage{float}
% \usepackage{url}
% \usepackage[normalem]{ulem}
% \lstset{
% 	basicstyle=\ttfamily,
% 	mathescape
% }
% \usepackage{comment}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm  
% \renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm 
% \usepackage{amsmath}
% \usepackage{epsfig}
% \usepackage{booktabs}
% \usepackage{lipsum}
% \usepackage{array}
% \usepackage{bbding} 
% \usepackage{setspace}

% \newsavebox{\measurebox}


% %%
% %% Submission ID.
% %% Use this when submitting an article to a sponsored event. You'll
% %% receive a unique submission ID from the organizers
% %% of the event, and this ID should be used as the parameter to this command.
% %%\acmSubmissionID{123-A56-BU3}

% %%
% %% For managing citations, it is recommended to use bibliography
% %% files in BibTeX format.
% %%
% %% You can then either use BibTeX with the ACM-Reference-Format style,
% %% or BibLaTeX with the acmnumeric or acmauthoryear sytles, that include
% %% support for advanced citation of software artefact from the
% %% biblatex-software package, also separately available on CTAN.
% %%
% %% Look at the sample-*-biblatex.tex files for templates showcasing
% %% the biblatex styles.
% %%

% %%
% %% The majority of ACM publications use numbered citations and
% %% references.  The command \citestyle{authoryear} switches to the
% %% "author year" style.
% %%
% %% If you are preparing content for an event
% %% sponsored by ACM SIGGRAPH, you must use the "author year" style of
% %% citations and references.
% %% Uncommenting
% %% the next command will enable that style.
% %%\citestyle{acmauthoryear}


% % DOI

% %\newdef{definition}{Definition}
% %\newdef{cond}{Condition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% % \newtheorem{proof}{Proof}
 
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \newcommand{\Paragraph} [1] {\smallskip\noindent{\bf #1. }}
% \newcommand{\red}[1]{\textcolor{red}{#1}}
% \newcommand{\blue}[1]{\textcolor{blue}{#1}}

% \newcommand{\lgl}[1]{\textcolor{blue}{#1}}
% \newcommand{\zyf}[1]{\textcolor{orange}{#1}}
% \newcommand{\zwx}[1]{\textcolor{blue}{#1}}
% \newcommand{\resp}[1]{\textcolor{magenta}{#1}}
% \newcommand{\pzs}[1]{\textcolor{cyan}{#1}}
% \newcommand{\wzy}[1]{\textcolor{magenta}{#1}}
% \newcommand{\zxj}[1]{\textcolor{green}{#1}}
% \newcommand{\hz}[1]{\textcolor{red}{HZ: #1}}

% \newcommand{\oursys}{\texttt{CCaaS}\xspace}
% \newcommand{\kw}[1]{{\ensuremath {\mathsf{#1}}}\xspace}
% \newcommand{\csn}{\kw{csn}}
% \newcommand{\sen}{\kw{sen}}
% \newcommand{\lsn}{\kw{lsn}}
% \newcommand{\cen}{\kw{cen}}
% \newcommand{\RR}{\kw{RR}}
% \newcommand{\RC}{\kw{RC}}
% \newcommand{\SI}{\kw{SI}}

% \newcommand{\crdb}{\texttt{CRDB}\xspace}
% \newcommand{\calvin}{\texttt{Calvin}\xspace}
% \newcommand{\leveldb}{\texttt{LevelDB}\xspace}
% \newcommand{\hbase}{\texttt{HBase}\xspace}
% \newcommand{\tidb}{\texttt{TiDB}\xspace}
% \newcommand{\foundationdb}{\texttt{FoundationDB}\xspace}

% \newcommand{\ie}{\emph{i.e.,}\xspace}
% \newcommand{\eg}{\emph{e.g.,}\xspace}
% \newcommand{\wrt}{\emph{w.r.t.}\xspace}
% \newcommand{\aka}{\emph{a.k.a.}\xspace}
% \newcommand{\kwlog}{\emph{w.l.o.g.}\xspace}
% \newcommand{\st}{\emph{s.t.}\xspace}
% \newcommand{\etc}{\emph{etc.}\xspace}

% % Include information below and uncomment for camera ready (sigmod)
% %\copyrightyear{2020}
% %\acmYear{2020}
% %\setcopyright{acmcopyright}
% %\acmConference[SIGMOD'20]{Proceedings of the 2020 ACM SIGMOD International Conference on Management of Data}{June 14--19, 2020}{Portland, OR, USA}
% %\acmBooktitle{Proceedings of the 2020 ACM SIGMOD International Conference on Management of Data (SIGMOD'20), June 14--19, 2020, Portland, OR, USA}
% %\acmPrice{15.00}
% %\acmDOI{10.1145/3318464.3389712}
% %\acmISBN{978-1-4503-6735-6/20/06}

% \begin{document}

% % whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
% \pagestyle{plain}
% \clearpage
% \setcounter{page}{1}

% \renewcommand{\shortauthors}{}
% %don't want date printed
% % \date{}

% % ****************** TITLE ****************************************

% \title{Concurrency Control as a Service: A Three-Layer Decoupled Database Architecture}
% % \title{Concurrency Control as a Service: A Three-Layer Cloud-Native Database Architecture}

% %\author{Weixing Zhou$^{\dagger}$, Qi Peng$^{\dagger}$, Zijie Zhang$^{\S}$, Yanfeng Zhang$^{\dagger}$, Yang Ren$^{\S}$, Sihao Li$^{\S}$, Guo Fu$^{\dagger}$, Yulong Cui$^{\dagger}$, Qiang Li$^{\S}$, Caiyi Wu$^{\dagger}$, Shangjun Han$^{\dagger}$, Shengyi Wang$^{\dagger}$, Guoliang Li$^{\ddagger}$, Ge Yu$^{\dagger}$}
% %\affiliation{
% % \institution{$\dagger$ Northeastern University, China, $\S$ Huawei Technology Co., Ltd, $\ddagger$ Tsinghua University, China}}
% %\email{}

% \begin{abstract}
% % Most of the state-of-the-art cloud-native databases simply decouple their systems into a execution and a storage layer to utilize the disaggregated computing and storage resources. 
% % However, transaction concurrency control (CC) focuses on resolving transaction conflicts, which requires compute resources to handle concurrent conflicts and has limited scaling capabilities due to coordination overhead. The resource requirement of CC is neither consistent with transaction execution, which allows free scaling, nor consistent with data storage, which requires huge storage space. Coupling CC with either execution or data storage limits the performance and elasticity.
% Many modern cloud-native databases employ disaggregated architectures, separating execution and storage layers to scale resources independently. This design make the transaction concurrency control (CC) a critical bottleneck, which demands significant computing resources and struggles to scale due to the overhead of coordination during concurrent conflict resolution. Coupling CC with either the execution or storage layer limits performance and elasticity, as CC's resource requirements do not align with the free scaling of transaction execution or the low, storage-bound resources of data storage layers.

% This paper proposes Concurrency Control as a Service ({\oursys}), which decouples CC from databases, allowing connections to a variety of execution and storage engines. 
% By using {\oursys}, we architect an execution-CC-storage three-layer decoupled database.
% Each layer can be independently scaled and upgraded to achieve high resource utilization and development agility.
% With {\oursys}: 1) NoSQL databases can be empowered with ACID transaction processing capability, 2) multiple standalone transaction processing engine instances can be incorporated to support multi-master distributed transaction processing for horizontal scalability, 3)  multiple execution engines with different data models can be integrated to support cross-model transactions.
% Existing cloud-native databases can be revolutionized with {\oursys} to achieve high elasticity, scalability, and high performance.
% Results show that {\oursys} achieves 4.7-8.5 times higher throughput and 4.9-5.8 times lower latency than state-of-the-art cloud-native databases under YCSB and TPC-C workloads.

% \end{abstract}

% % Use the following at camera-ready time to suppress page numbers. (osdi)
% % Comment it out when you first submit the paper for review.
% % \thispagestyle{empty}

% %%
% %% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% %% Please copy and paste the code instead of the example below.
% %%
% % \begin{CCSXML}
% % <ccs2012>
% %     <concept>
% %     <concept_id>10002951.10002952.10003190.10003195.10010838</concept_id>
% %        <concept_desc>Information systems~Relational parallel and distributed DBMSs</concept_desc>
% %        <concept_significance>500</concept_significance>
% %     </concept>
% %  </ccs2012>
% % \end{CCSXML}
% % 
% % \ccsdesc[500]{Information systems~Relational parallel and distributed DBMSs}

% \keywords{Cloud-native database architecture; multi-master database; transaction processing; concurrency control;}

% % \ccsdesc[500]{Computer systems organization~Dependable and fault-tolerant systems and networks}

% % %%
% % %% Keywords. The author(s) should pick words that accurately describe
% % %% the work being presented. Separate the keywords with commas.
% % \keywords{Geo-Distributed Replication, Fault Tolerance, Consensus}

% %%
% %% This command processes the author and affiliation and title
% %% information and builds the first part of the formatted document.
% \maketitle

% \input{1 intro}
% \input{2 case}
% % \input{2 background}
% \input{3 system}
% \input{4 trans}
% \input{5 implementation}
% \input{6 discuss}
% \input{7 expr}
% \input{8 related}

% % \begin{acks}
% % The work is supported by the National Natural Science Foundation of China (62072082, U2241212, 62202088, 62232009, 61925205, 62137001, 62272093), the National Social Science Foundation of China (21\&ZD124), CCF-Huawei Populus euphratica Innovation Research Funding (CCF-HuaweiDB2022003), the Fundamental Research Funds for the Central Universities (N2216012, N2216015), Huawei, TAL education, and Beijing National Research Center for Information Science and Technology (BNRist). Yanfeng Zhang is the corresponding author.
% % \end{acks}


% % \balance

% % \bibliographystyle{ACM-Reference-Format}
% % \bibliography{vldb_sample}



% % {\footnotesize \bibliographystyle{acm}
% \bibliographystyle{ACM-Reference-Format}
% \bibliography{all}


% % \theendnotes



% \end{document}

